A plausible Parametrization of Modal Basis for Dynamical Systems Analysis

In the field of solid dynamics, knowing the corresponding modal basis of the system is capital, in order to improve design with respect to a desired dynamical behavior, such as avoiding natural frequencies at specific values or designing mechanical systems that can account for desired frequency spectrum. However, the determination of the modal basis involve the resolution of an eigenvalue problem, which can be expensive to perform for large systems, especially when dealing with a optimization of a parametric system design. In the present work, we propose to determine the parametrization of modal basis by considering an advanced Deep Learning technique based on the Rank Reduction AutoEncoder (RRAE). The RRAE is based on an autoencoder whose latent space is constrained through a truncated Singular Value Decomposition (SVD) approximation. This formulation enables the latent space to capture the dominant features of the data efficiently. As a result, the autoencoder is guided toward learning the underlying physical behavior represented across the dataset, mitigating overfitting and spurious predictions. The main idea consists of identifying a reduced parameter space using the RRAE for the first eigenvector, while the remaining modes are subsequently reconstructed through neural networks that take the same reduced parameter space as input, thereby coupling all modes in a nonlinear parametric framework. The proposed architecture is validated through the parametrization of the modal basis in 1D and 2D problems.

==> Notations.tex <==
%%%% Notations %%%%

% Macro/micro
\newcommand{\fM}{H}
\newcommand{\fm}{h}

\newcommand{\tM}{t_{M}}
\newcommand{\tm}{t_{m}}




\newcommand{\pgdtinit}{\nu}

\newcommand{\pgdsinit}{\phi}


% Number of sensors for each direction:

\newcommand{\Nxs}{n_{s,x}}
\newcommand{\Nys}{n_{s,y}}


% Classic sets:
\newcommand{\Ree}{\mathbb{R}} % Real


% Domaines
\newcommand{\DS}{\mathrm{\Omega}}             % Domaine spatial
\newcommand{\DT}{{I}}                  % Domaine temporel

% Reduced time domain:
\newcommand{\DTtrain}{I^{\text{train}}}

% Reduced time domain:
\newcommand{\DTex}{I^{\text{ex}}}

% Reduced time domain:
\newcommand{\DTexr}{\DT^{\text{ex}}_{\text{red}}}

% Pressures:
\newcommand{\pr}{p}

% Parameters:
\newcommand{\param}{\bar{t}}


% Arrival times:
\newcommand{\vat}{\SDvect{T}}
\newcommand{\at}{T}




% sPGD approx arrival time:
\newcommand{\PGDat}{T_{\PGDm}}
\newcommand{\PGDati}{T_{\PGDm_{i}}}

% sPGD of the ignorance
\newcommand{\PGDigi}{\Delta T_{\PGDmig_{i}}}


% end Arrival times.





\newcommand{\vx}{\vect{x}} % x vector
\newcommand{\vp}{\vect{\param}}
\newcommand{\vpi}{\hat{\vect{\param}}}
\newcommand{\vpo}{\vect{\param}_{\text{out}}}


\providecommand{\abs}[1]{\lvert#1\rvert}

% PGD functions:
\newcommand{\PGDf}{X} 
\newcommand{\X}{\PGDf_{1}} 
\newcommand{\Y}{\PGDf_{2}} 
\newcommand{\varX}{\Tilde{t}_M} 
\newcommand{\varY}{\param_{2}} 




\newcommand{\pmv}{\hspace{0.5mm}} % producto entre matrices y vectores.
%\hspace{0.5mm}

























\newcommand{\Span}[1]{\mbox{span} #1}


%% Spaces of continuous solutions

\newcommand{\Su}{\mathcal{U}} % \mathscr{U}     % 
\newcommand{\SuS}{\Su^S}  % Spatial problem 
\newcommand{\SuT}{\Su^T}  % Temporal problem
\newcommand{\Ssobolev}{\mathcal{H}_1}
\newcommand{\SuP}{\DS^{P}}  % Parametric space:

\newcommand{\SuTd}{\Su^{\breve{T}}}
\newcommand{\Ssig}{\mathcal{F}}        % Espace des solutions en contrainte


\newcommand{\PGDm}{m} % Mode number notation.

\newcommand{\PGDminit}{m_{\text{init}}} % Mode number notation.


%%% Notations %%%




%%%%%%%%%%%%%%%%%%%



\newcommand{\test}[1]{{#1}^{\ast}}


% Espaces de solutions (Continues)
\newcommand{\Eu}{\mathscr{U}}        % Espace des solutions en déplacement
%\newcommand{\Eu}{\mathcal{U}} \mathscr{U}
\newcommand{\EuS}{\Eu^S}             % Problème spatial
\newcommand{\EuT}{\Eu^T}             % Problème temporel
%\newcommand{\EuTd}{\Eu^{\breve{T}}}
\newcommand{\EuP}{\Eu^P}             % Problème paramétrique
\newcommand{\Esig}{\mathcal{F}}        % Espace des solutions en contrainte
\newcommand{\EsigS}{\Esig^S}
\newcommand{\EsigT}{\Esig^T}
\newcommand{\Eeps}{\mathcal{E}} 	% Espace des deformations
\newcommand{\EepsS}{\Eeps^S}
\newcommand{\EepsT}{\Eeps^T}
\newcommand{\Esobolev}{\mathscr{H}_1}
\newcommand{\Elagrange}{\mathscr{L}}





\newcommand{\EGamma}{\boldsymbol{\Gamma}} % Delta
\newcommand{\EAd}{\boldsymbol{A_{d}}} % Delta






\newcommand{\IV}{{X}}
\newcommand{\SF}{\mathcal{F}}



% Définition de l'environnement parboxed : paragraphes encadrés [framed]
\newenvironment{parboxed}[1][black]
  {\def\FrameCommand{\fboxsep=\FrameSep\fcolorbox{#1}{white}}%
    \MakeFramed {\advance\hsize-\width \FrameRestore}}
  {\endMakeFramed}

% Définition de l'environnement colorboxed : paragraphes en couleur [framed]
\newenvironment{colorboxed}[2][black]
  {\def\FrameCommand{\fboxsep=\FrameSep\fcolorbox{#1}{#2}}%
    \setlength\fboxrule{0pt}
    \MakeFramed {\advance\hsize-\width \FrameRestore}}
  {\endMakeFramed}


% Environnement probleme [amsthm]
\theoremstyle{definition}
\newtheorem{prob}{\textsc{Problem}}%[section]
\newenvironment{probleme}[1][htbp]{
		\begin{parboxed}
		    \begin{prob}
	}{
		    \end{prob}
		\end{parboxed}
	}


% Tableaux a utiliser dans un environnement equation ou align
% format de type \forall    equation 
\newcommand{\tableq}[2]{
\hspace{0.01\hsize}\makebox[0.2\hsize][l]{${#1}$} \hspace{-0.17\hsize}\makebox[0.88\hsize][c]{$\displaystyle #2$}%\hspace{-0.02\hsize}
}

\newcommand{\ACC}[1]{\Big\{{#1}\Big\}}


% General material parameters
\newcommand{\VarX}{\mathcal{X}} 	% Primal variables / Internal variables
\newcommand{\VarY}{\mathcal{Y}} 	% Dual variables / Thermodynamic forces

% Relations de comportement generales
\newcommand{\RdC}{\mathcal{R}}


\newcommand{\rmDelta}{\mathrm{\Delta}} % Delta



\newcommand{\eqtext}[1]{{\vspace{2mm} \noindent {#1}}}


\newcommand{\com}{,} % dot product


\newcommand{\dotp}{\cdot} % dot product

\newcommand{\p}{\hspace{0.5mm}} % producto entre matrices y vectores.
%\hspace{0.5mm}

% Final solution LATIN:

\newcommand{\SOLex}{\bar{\SOL}}



\newcommand{\vpnop}{\bar{\Upsilon}}





\newcommand{\tdof}{n_{T}}
\newcommand{\sdof}{n_{S}}





\newcommand{\med}{me}
\newcommand{\cra}{cr}


%\newcommand{\rhoc}{\rho_{c}}
%\newcommand{\rhop}{\rho_{p}}

\newcommand{\rhoc}{\rho}
\newcommand{\rhop}{\rho}


\newcommand{\ind}{i}




% Function figure:
%\newcommand{\Figure}[1]{\mathit{{#1}}}





% Notation matrices:


% Vector notation:
\newcommand{\vect}[1]{\underline{{#1}}} 
%\newcommand{\vect}[1]{\mathit{{#1}}} 

% Tensor of 2nd order
\newcommand{\ctens}[1]{\underline{\underline{{#1}}}} 
%\newcommand{\ctens}[1]{\mathit{{#1}}} 



% Representation semi-discrete vector:
\newcommand{\SDvect}[1]{%
            \underline{\boldsymbol{\mathbf{%
                \mathit{#1}
            }}}
}


% Representation discrete vector:
\newcommand{\Dvect}[1]{%
            \underline{\boldsymbol{\mathbf{%
                {#1}
            }}}
}

% Representation semi-discretize tensor:
\newcommand{\SDtens}[1]{%
            \underline{\underline{\boldsymbol{\mathbf{%
                \mathit{#1}
            }}}}
}

 

% Representation discrete tensor:
\newcommand{\Dtens}[1]{%
            \underline{\underline{\boldsymbol{\mathbf{%
                {#1}
            }}}}
}
\begin{comment}
\newcommand{\Dtens}[1]{%
            \boldsymbol{\mathbf{%
                {#1}
            }}
}
\end{comment}



% Tensor of 4 order
%\newcommand{\ctens4}[1]{\mathit{{#1}}} 
\newcommand{\ctensd}[1]{\mathbb{{#1}}}
%\newcommand{\ctensd}[1]{\underline{\underline{\underline{\underline{\mathbb{{#1}}}}}}}



% Representation discrete 4 order tensor:
\newcommand{\SDtensd}[1]{%
            \underline{\underline{\underline{\underline{\boldsymbol{{%
                {#1}
            }}}}}}
}
\newcommand{\Dtensd}[1]{%
            \underline{\underline{\underline{\underline{\boldsymbol{\mathbf{%
                {#1}
            }}}}}}
}
\begin{comment}
\newcommand{\Dtensd}[1]{%
            \boldsymbol{\mathbf{%
                {#1}
            }}
}
\end{comment}




%% End Notation matrices. 




% Equality:
\newcommand{\eq}{ \ = \ }


%%%%%%%%% REFERENCE PROBLEM:

% Tangent operator tensor:
\newcommand{\Tanop}{\ctensd{T}_{op}}

% Discretized Matrix 	associated to the tanget behavior:
\newcommand{\SOP}{\SDtens{S}}


% Newmark:
\newcommand{\Ngamma}{\gamma_{s}}
\newcommand{\Nbeta}{\beta_{s}}



% Nonlinear function:
\newcommand{\NLfunc}{\mathcal{J}}
% Acceleration funct:
\newcommand{\Acc}{\mathcal{L}}

% Incremental sol
\newcommand{\sol}{s}
% Index of incremental iteration:
\newcommand{\Ii}{n}
% Strain tensor:
\newcommand{\eps}{\varepsilon}




% Reduced matrices:
\newcommand{\Mred}[1]{\bar{#1}}


% Bilinear form and Linear form:
\newcommand{\BLnot}[1]{\mathpzc{#1}}
\newcommand{\Rnot}[1]{\mathcal{#1}}

% No discrete:
\newcommand{\A}{ \BLnot{A} }
\newcommand{\B}{ \BLnot{B} }

\newcommand{\SDR}{ \SDvect{R} } % semi discretized residual

% Discrete way:
\newcommand{\DA}{ \Dtensd{A} }
\newcommand{\DB}{ \Dtens{B} }
\newcommand{\DR}{ \Dtens{R} } % discretized residual



% Riesz representation:
\newcommand{\RA}{ \Rnot{A} }
\newcommand{\RB}{ \Rnot{B} }




\newcommand{\normi}[1]{\left\|{#1}\right\|}

\newcommand{\normiS}[1]{\left\|{#1}\right\|_{\DS}}
\newcommand{\normiT}[1]{\left\|{#1}\right\|_{\DT}}



% General space-time norm:
\newcommand{\norm}[1]{\left|\left|\left| #1 \right|\right|\right|}
%\newcommand{\norm}[1]{\big|\big|\big|#1\big|\big|\big|}





%%%% Factor of resize for intro MS:

\newcommand{\fs}{0.65}




%%%% Material constants:

% Constant modal damping ratio
\newcommand{\md}{\epsilon}

% General damping tensor:
\newcommand{\Damp}{\ctensd{D}}

% General hooke tensor:
\newcommand{\Hooke}{\ctensd{K}}

% Young modulus:
\newcommand{\Ym}{E}

% Poisson coeficient:
\newcommand{\Pc}{\nu}



%% Isotropic damage:

%\newcommand{\HookeC}{\Hooke_{c}}
\newcommand{\HookeC}{\Hooke}

% Young modulus:
\newcommand{\Ymc}{\Ym}
% Poisson coeficient:
\newcommand{\Pcc}{\Pc}


% Brittleness coefficient
\newcommand{\Ad}{A_{d}}
% Damage delay time constant
\newcommand{\dd}{\tau_{c}}
% Damage delay exp. constant
\newcommand{\ddexp}{a}
% Crack-closure dimensionless constant
\newcommand{\cc}{a_{c}}


%% Elasto-visco-plasticity:

%\newcommand{\HookeP}{\Hooke_{p}}
%\newcommand{\Ymp}{\Ym^{p}}
%\newcommand{\Pcp}{\Pc^{p}}


\newcommand{\HookeP}{\Hooke}
\newcommand{\Ymp}{\Ym}
\newcommand{\Pcp}{\Pc}


\newcommand{\Rinf}{R_{\infty}}
\newcommand{\Cvp}{C}
\newcommand{\avp}{a}
\newcommand{\bvp}{b}
\newcommand{\nvp}{n_{s}}
\newcommand{\kvp}{k}
\newcommand{\Kvp}{K}




%%%% end Material constants:






% Force:
\newcommand{\f}{f}
% Semi discretized force:
\newcommand{\SDf}{\SDvect{\f}}
% Discretized force:
\newcommand{\Df}{\Dtens{\f}}


% Force at the modal approximation: 
% Semi discretized force:
\newcommand{\SDfm}{\SDvect{\f}_{\id}}
% Discretized force:
\newcommand{\Dfm}{\Dtens{\f}_{\id}}


%%%%%%%%% END REFERENCE PROBLEM:




%%%%%%%%%%  NOTATION OVERVIEW : %%%%%%%%

% eingenvalue pod:
\newcommand{\egvpod}{\varsigma}

% Space of low-rank approximations:
\newcommand{\Sr}{\mathcal{R}} % \mathscr{U}    


% POD symbol:
\newcommand{\podi}{\triangledown}
\newcommand{\Dpodi}{\blacktriangledown}


% PGD symbol:
\newcommand{\pgdi}{\vartriangle}
\newcommand{\Dpgdi}{\blacktriangle}


% Posteriori norm:
\newcommand{\Jpo}{J^{\podi}}
% discretized
\newcommand{\DJpo}{\boldsymbol{J}^{\Dpodi}}                   



% A Priori norm:
\newcommand{\Jap}{J^{\pgdi}}
% discretized 
\newcommand{\DJap}{\boldsymbol{J}^{\Dpgdi}}



% reduce order model field notation:
\newcommand{\red}[1]{{#1}^{rb}}

% Low rank decomposition:
% Space function:
\newcommand{\pgds}{w}


% Matrix of spatial vectors that constain the modes:
\newcommand{\Mpgds}{W}

% Matrix of temporal function that contains the modes:
\newcommand{\Mpgdt}{\Lambda}







%% CRBM:



% Paramter
\newcommand{\pcr}{\theta} % Parameter

% Domaine des parametres
\newcommand{\DP}{I_{\pcr}}             

\newcommand{\Manf}{\mathcal{M}}         % Manifold
\newcommand{\Manffem}{\mathcal{M}_{h}}  % Manifold discret


\newcommand{\mop}{\BLnot{m}}
\newcommand{\dop}{\BLnot{d}}
\newcommand{\kop}{\BLnot{k}}
\newcommand{\fop}{\BLnot{f}}



\newcommand{\lcr}{\BLnot{l}}
\newcommand{\acr}{\kop}
\newcommand{\mcr}{\mop}
\newcommand{\fcr}{\fop}
\newcommand{\rcr}{\BLnot{R}}
\newcommand{\scr}{\BLnot{s}}


\newcommand{\urb}{\red{\vect{u}}}
\newcommand{\srb}{\red{\scr}}


% Error estimators:
\newcommand{\ncrEN}{
\eta_{\text{en}}(\pcr)}
\newcommand{\ncrS}{
\eta_{\text{s}}(\pcr)}
\newcommand{\ncrSREL}{
\eta_{\text{s,rel}}(\pcr)}

% Effectiveness:
\newcommand{\effEN}{
\text{eff}_{\text{en}}(\pcr)}
\newcommand{\effS}{
\text{eff}_{\text{s}}(\pcr)}
\newcommand{\effSREL}{
\text{eff}_{\text{s,rel}}(\pcr)}



% Important Constants:
\newcommand{\gam}{\mathpzc{\gamma}} % Constant error
\newcommand{\alf}{\mathpzc{\alpha}} % Constant error
\newcommand{\alfLB}{\alf_{\text{LB}}}



%% APHRM:

% Selection matrix for the reduce domain:
\newcommand{\rM}{\Pi} % Parameter


% Annexes:  
\newcommand{\Xpod}{\SDtens{X}}
\newcommand{\xpod}{\SDvect{x}}
\newcommand{\Ypod}{\SDtens{Y}}
\newcommand{\ypod}{\SDvect{y}}
\newcommand{\Wpod}{\SDtens{W}}

\newcommand{\Npod}{N_{v}}
\newcommand{\Nstate}{\PGDm}



% SVD:
\newcommand{\Usvd}{\SDtens{U}}
\newcommand{\Vsvd}{\SDtens{V}}
\newcommand{\Ssvd}{\SDtens{\Sigma}}

% Eigenvalue Decomp:
\newcommand{\Seig}{\SDtens{\Lambda}}

% Error:
\newcommand{\epod}{\xi}

% Sample mean:
\newcommand{\SM}{E_{\ypod}}



% END OVERVIEW ROM:











%% Shape functions:
\newcommand{\sfS}{\chi}
\newcommand{\sfSv}{\vect{\sfS}}

\newcommand{\sfT}{\psi}
%\newcommand{\sfTvT}{\vect{\sfT}^{T}(t)}
\newcommand{\sfTv}{\vect{\sfT}}
\newcommand{\sfTvf}{\vect{\psi}}
 

% Macro shape function:
\newcommand{\sfTM}{\Psi}
\newcommand{\sfTMv}{\vect{\sfTM}}



% Discrétisation (FEM)
\newcommand{\discrS}[1]{{#1}^{h}}
% Discrétisation (FEM space-time)
\newcommand{\discrST}[1]{{#1}^{\mathcal{N}}}



\newcommand{\ifem}{\mathcal{N}} % index fem
\newcommand{\dt}{\rmDelta t} % size of time on an fem element finer discretization:

% D contraccion.
\newcommand{\Dim}{\mathsf{D}}
\newcommand{\xD}{ \overset{\Dim}{.} }



\newcommand{\Par}{\medskip\par}
\newcommand{\prth}[1]{({#1})} % little parenthesis ()
\newcommand{\Prth}[1]{\left({#1}\right)} % big parenthesis ()
\newcommand{\Prthc}[1]{\left[{#1}\right]} % big parenthesis []
\newcommand{\prtha}[1]{\langle {#1} \rangle}




% Classic sets:
\newcommand{\R}{\mathbb{R}} % Real
\newcommand{\C}{\mathbb{C}} % Complex
\newcommand{\N}{\mathbb{N}} % Natural 



\newcommand{\Macro}{M}
\newcommand{\DTM}{\DT^{\Macro}}                  % Domaine temporel Macro
\newcommand{\DTm}{\DT}                  % Domaine temporel micro



\newcommand{\DTd}{\breve{\DT}} % Temporal discontinuous domain.
\newcommand{\DTk}{\breve{\DT}_{k}} % Temporal disco domain on element k.
%\newcommand{\DF}{J}



%% Discretized space solutions:

% Espace des solutions en déplacement

\newcommand{\Sufem}{\Su_h} %
\newcommand{\SufemS}{\Su_h^S}             % Problème spatial
\newcommand{\SufemT}{\Su_{\rmDelta  t}^T}     

%% Discretized reduced space solution:
\newcommand{\ir}{r}
\newcommand{\rSufemS}{\Su_{\PGDm}^S}             % Problème spatial



% Spatial DOFs:
\newcommand{\nS}{n_S}             
% N of DOFs in time:
\newcommand{\nT}{n_T}            
% N of elements in time:
\newcommand{\NT}{N_T}              

% N of elements in space:
\newcommand{\NS}{N_S}              




% N of integration points in time:
\newcommand{\Npgt}{n_{t,g}}
% N of DOFs parametric:
\newcommand{\nP}{n_P}


% Discretized spaces:

\newcommand{\RnS}{\R^{\nS}}
\newcommand{\RnT}{\R^{\nT}}
\newcommand{\RnST}{\RnS \otimes \RnT}
%\newcommand{\RnSm}{\prth{\R^{\nS}}^\m}
%\newcommand{\RnTm}{\prth{\R^{\nT}}^\m}











%%%%%%%%%% LATIN-PGD %%%%%%%%%%%%%%%%%

% Initial condition sub index notation.
\newcommand{\init}{{in}}




% Constitutive relation errors:


\newcommand{\CREc}{J}
\newcommand{\CREp}{J^{p}}
\newcommand{\CREa}{J^{\alpha}}
\newcommand{\CREr}{J^{\bar{r}}}








\newcommand{\SDdc}{\mathbb{G}}
\newcommand{\SDac}{\mathbb{A}}

\newcommand{\SAd}{\boldsymbol{A_d}}
\newcommand{\SGam}{\boldsymbol{\Gamma}}

\newcommand{\SOL}{\mathcal{S}}






%% LATIN Modal base approx:

\newcommand{\cd}{c_{d}} % modal base index



\newcommand{\id}{d} % modal base index

\newcommand{\Fcr}{\ctens{f}^{cr}} 



% Corrective modal base:

% hat corresponding to the modal base associated to the corrective equation:
\newcommand{\hatc}[1]{ \tilde{#1} }


\newcommand{\Smbc}{\hatc{\vect{\phi}}} % Modal base space functions.
\newcommand{\TSmbc}{\hatc{\ctens{\Phi}}} % Modal base displacement functions.
\newcommand{\Tmbc}{\hatc{\upsilon}} % modal base temporal functions.

\newcommand{\SDSmbc}{\hatc{\SDvect{\phi}}} % Semi discrete Modal base displacement.
\newcommand{\SDTSmbc}{\hatc{\SDtens{\Phi}}} % Semi discrete Modal base displacement.

% Temporal function and total temporal function of the elastic problem:
\newcommand{\Tec}{\hatc{\SDvect{\upsilon}}}
\newcommand{\TecT}{\hatc{\SDvect{\Upsilon}}}


% end corrective modal base.







% Elastic modal base:

\newcommand{\nmb}{m_{b}} % number of modes of the modal base.


\newcommand{\Smb}{\vect{\phi}} % Modal base space functions.
\newcommand{\TSmb}{\ctens{\Phi}} % Modal base displacement functions.
\newcommand{\SDSmb}{\SDvect{\phi}} % Semi discrete Modal base displacement.
\newcommand{\SDTSmb}{\SDtens{\Phi}} % Semi discrete Modal base displacement.




\newcommand{\Tmb}{\upsilon} % modal base temporal functions.
\newcommand{\TTmb}{\Upsilon} % modal base temporal functions.


% Discretized Temporal function and total temporal function of the elastic problem:
\newcommand{\Te}{\SDvect{\Tmb}}
\newcommand{\TeT}{\SDtens{\TTmb}}

% End elastic modal base.






% INITIAL SOLUTION:

% elastic index
\newcommand{\ie}{0}

\newcommand{\uo}{\vect{u}_{\ie}}
\newcommand{\SDuo}{\SDvect{u}_{\ie}}
\newcommand{\tSDuo}{\dot{\SDvect{u}}_{\ie}}
\newcommand{\ttSDuo}{\ddot{\SDvect{u}}_{\ie}}

\newcommand{\Duo}{\Dtens{u}_{\ie}}

\newcommand{\sigmao}{\ctens{\sigma}_{\ie}}
\newcommand{\epso}{\ctens{\varepsilon}_{\ie}}







% Quasi-static and dynamics displacements:
\newcommand{\uq}{\vect{u}_{\ie,\iq}}
\newcommand{\ud}{\vect{u}_{\ie,\id}}

% semi discretized:
\newcommand{\SDuq}{\SDvect{u}_{\ie,\iq}}
\newcommand{\SDud}{\SDvect{u}_{\ie,\id}}

% first derivative:
\newcommand{\tSDuq}{\dot{\SDvect{u}}_{\ie,\iq}}
\newcommand{\tSDud}{\dot{\SDvect{u}}_{\ie,\id}}

% second derivative:
\newcommand{\ttSDuq}{\ddot{\SDvect{u}}_{\ie,\iq}}
\newcommand{\ttSDud}{\ddot{\SDvect{u}}_{\ie,\id}}


% Discretized fields:
\newcommand{\Duq}{\Dtens{u}_{\ie,\iq}}
\newcommand{\Dud}{\Dtens{u}_{\ie,\id}}


% Matrix and vector:
\newcommand{\Mp}{\SDtens{Q}}
\newcommand{\Rp}{\SDtens{\mathcal{R}}}
\newcommand{\Fp}{\SDvect{F}}
\newcommand{\fp}{\SDvect{f}}



%\nmb
% Total matrices and vector:
\newcommand{\MpT}{\bar{\SDtensd{Q}}}
\newcommand{\RpT}{\bar{\SDtensd{R}}}
\newcommand{\FpT}{\bar{\SDtens{f}}}
\newcommand{\fpT}{\bar{\SDtens{f}}}


% END INITIAL SOLUTION




% Stagnation of for the update stage:
\newcommand{\pgderror}{\zeta_{PGD}}



% Stagnation of for the update stage:
\newcommand{\uperror}{\zeta_{up}}


% Error of the LATIN method:
\newcommand{\LATINerror}{\xi}

% Strain and stress elastic tensors:
\newcommand{\sige}{\ctens{\sigma}^{e}}
\newcommand{\epse}{\ctens{\varepsilon}^{e}}



\newcommand{\I}{\SDtens{I}} % Identity matrix.


% General search directions:
\newcommand{\SDa}{\mathit{G}}
\newcommand{\SDd}{\mathit{A}}

% Search directions concrete:
\newcommand{\SDaC}{\SDa}
\newcommand{\SDdC}{\SDd}


% Search directions vp:
\newcommand{\SDaP}{\SDa}
\newcommand{\SDdP}{\SDd}


% Tangent operator:
\newcommand{\Top}{\ctensd{H}}


%1) Ascent tangent operator: direction): (viscoplasticity)
\newcommand{\Topa}{\hat{\Top}}
% descent tangent operator:
\newcommand{\Topd}{\Top}


%1) Tangent operator stress(descent search direction): (viscoplasticity)
\newcommand{\Tops}{\Top_{\sigma}}


% Tangent operator strain(ascent search direction): (Concrete material)
\newcommand{\Topea}{\hat{\Top}_{\varepsilon}}

%1) Tangent operator strain  (descent search direction): (Concrete material)
\newcommand{\Tope}{\Top_{\varepsilon}}



%2) Tangent operator internal variables:
\newcommand{\Topza}{\hat{\Top}_{Z}}

\newcommand{\Topz}{\Top_{Z}}
\newcommand{\Topb}{\Top_{\beta}}
\newcommand{\Toprbar}{H_{\bar{R}}}







% Left matrix continuity:
\newcommand{\LM}{\SDtens{\mathcal{L}}}

% Right matrix continuity:
\newcommand{\RM}{\SDtens{\mathcal{R}}}




\SetKwInOut{Parameter}{Parameters}

\newcommand{\utest}{\test{\vect{u}}}
\newcommand{\utestdt}{\test{\dot{\vect{u}}}}
\newcommand{\utestdtdt}{\test{\ddot{\vect{u}}}}


\newcommand{\Li}{n} % Latin index number iteration.

\newcommand{\Lii}{\ell} % Latin index number iteration.


% Parametric pgd:
\newcommand{\pgdp}{\pi}

% Space pgd displacement:
\newcommand{\pgdv}{\bar{\vect{\utest}}}  
% Space pgd displacement:
\newcommand{\pgdu}{\bar{\vect{u}}}  

\newcommand{\SDpgdu}{\bar{\SDvect{u}}}  


% Space pgd stress:
\newcommand{\pgdsig}{\bar{\ctens{\sigma}}}
% Space pgd plastic strain:
\newcommand{\pgdepsp}{\bar{\ctens{\varepsilon}}^{p}}
% Space pgd strain:
\newcommand{\pgdeps}{\bar{\ctens{\varepsilon}}}

% Residual functions LATIN:
\newcommand{\Lres}{{\ctens{\rmDelta}}}
\newcommand{\Lresc}{\Lres}
\newcommand{\Lresp}{\Lres}

\newcommand{\Lresi}{{\ctens{\rmDelta}}}
\newcommand{\Lresic}{\Lresi}
\newcommand{\Lresip}{\Lresi}






% Time function of the pgd decomposition:
\newcommand{\pgdt}{\lambda}

% Time function actualization part:
\newcommand{\tu}{\rmDelta \lambda }
% Derivative of the act time function:
\newcommand{\ttu}{\rmDelta \dot{\lambda}}



% Temporal discretized problems:

% Enrichment Matrix and Vector:
\newcommand{\Mt}{\SDtens{Q}}
\newcommand{\Ft}{\SDvect{f}}

% Actualization Matrix and Vector:
\newcommand{\up}{up}

\newcommand{\MT}{\SDtens{Q}_{\up}}
\newcommand{\FT}{\SDvect{f}_{\up}}

\newcommand{\LMT}{\LM_{\up}}
\newcommand{\RMT}{\RM_{\up}}



%Internal variables:

% Space functions:
\newcommand{\pgda}{\bar{\ctens{\alpha}}}
\newcommand{\pgdrbar}{\bar{\bar{r}}}

% Time functions 
\newcommand{\ta}{\lambda^{\alpha}}
\newcommand{\tta}{\dot{\lambda}^{\alpha}}
\newcommand{\trbar}{\lambda^{\bar{r}}}
\newcommand{\ttrbar}{\dot{\lambda}^{\bar{r}}}



% Residual functions LATIN:
\newcommand{\Lresa}{{\ctens{\rmDelta}}^{\alpha}}
\newcommand{\Lresrbar}{{\rmDelta}^{\bar{r}}}



% Time function actualization part:
\newcommand{\tua}{\rmDelta \lambda^{\alpha}}
% Derivative of the time function:
\newcommand{\ttua}{\rmDelta \dot{\lambda}^{\alpha}}

\newcommand{\turbar}{\rmDelta    \lambda^{\bar{r}}}
% Derivative of the time function:
\newcommand{\tturbar}{\rmDelta  \dot{\lambda}^{\bar{r}}}



% Semi discretized update functions:

\newcommand{\SDtu}{\rmDelta  \SDvect{\lambda} }

\newcommand{\SDtua}{\rmDelta  \SDvect{\lambda}^{\alpha} }

\newcommand{\SDturbar}{\rmDelta  \SDvect{\lambda}^{\bar{r}} }

% vector that contains all the semi discretized corrections:


\newcommand{\Ttu}{\Lambda} 


\newcommand{\SDTtu}{ \SDvect{\Lambda} }

\newcommand{\SDTtua}{ \SDvect{\Lambda}^{\alpha} }

\newcommand{\SDTturbar}{ \SDvect{\Lambda}^{\bar{r}} }




% Preliminary step: Space.
\newcommand{\SDUT}{\SDtens{U}}



%%%%%%% End LATIN-PGD



%%%%%%%%% % Multi-scale %%%%%%%%%%%%%%%%%


% Macro time interval:
\newcommand{\dT}{\rmDelta T}
\newcommand{\dTk}{\dT_{\is}}

% Number of cycles on the macro elements:
\newcommand{\Nc}{N_{c}}
\newcommand{\Nci}{N_{c,\is}}
\newcommand{\Nmc}{n_{c}} % number of micro cycles into a macro interval
\newcommand{\Nms}{n_{s}} % number of sub-modes


% Macro elements:
\newcommand{\NTm}{N_{\is}}

%% Theory of Signal

\newcommand{\iS}{s} % index to sub modes index. 

\newcommand{\ip}{p} % patch index. 
\newcommand{\ik}{k} % patch index. 

\newcommand{\inod}{\mathit{l}} % patch index. 
%\iota


\newcommand{\is}{\ell} % Index for the signal modes
\newcommand{\ms}{m_{s}} % seismic modes

\newcommand{\chp}{\tau} % characteristic period.
\newcommand{\chpk}{\chp_{\is}} % characteristic period sub k.


\newcommand{\sref}{s_{ref}} % reference signal
\newcommand{\saprox}{{s}} % Approx signal function
\newcommand{\smode}{\smod{\saprox}} % signal mode

\newcommand{\mTS}{{W}}
\newcommand{\resTS}{r}




% semi discretized amplitud macro:
\newcommand{\SDA}{\SDvect{A}}
\newcommand{\vn}{{n}}
\newcommand{\vF}{{f}}






% LATIN multiscale approach:

\newcommand{\re}{\text{R}}
\newcommand{\im}{\text{I}}



% Multi-scale sub temporal modes:
\newcommand{\smod}[1]{\bar{#1}}


%1) Operator R:
\newcommand{\Ro}{\SDtens{R}}

%2) Operator G:
\newcommand{\Go}{\SDtens{\hat{G}}}

% J functional.
\newcommand{\Ja}{J^{\alpha}}
\newcommand{\Jr}{J^{\bar{r}}}

% q functional
\newcommand{\q}{q}
\newcommand{\qa}{q^{\alpha}}
\newcommand{\qr}{q^{\bar{r}}}


% Macro functions admissibility:
\newcommand{\AR}{A^{\re}}
\newcommand{\AI}{A^{\im}}
\newcommand{\Ac}{A^{o}} % constant

\newcommand{\ARk}{\AR_{\is}}
\newcommand{\AIk}{\AI_{\is}}
\newcommand{\Ack}{\Ac_{\is}}



% Micro functions admissibility:

\newcommand{\hR}{h^{\re}}
\newcommand{\hI}{h^{\im}}

\newcommand{\hRk}{\hR_{\is}}
\newcommand{\hIk}{\hI_{\is}}

\newcommand{\thRk}{\dot{h}^{\re}_{\is}}
\newcommand{\thIk}{\dot{h}^{\im}_{\is}}



% Micro functions (LATIN) (Internal variables):

\newcommand{\haR}{h^{\re,\alpha}}
\newcommand{\haI}{h^{\im,\alpha}}
\newcommand{\thaR}{\dot{h}^{\re,\alpha}}
\newcommand{\thaI}{\dot{h}^{\im,\alpha}}

\newcommand{\haRk}{\haR_{\is}}
\newcommand{\haIk}{\haI_{\is}}
\newcommand{\thaRk}{\thaR_{\is}}
\newcommand{\thaIk}{\thaI_{\is}}



\newcommand{\hrR}{h^{\re,\bar{r}}}
\newcommand{\hrI}{h^{\im,\bar{r}}}
\newcommand{\thrR}{\dot{h}^{\re,\bar{r}}}
\newcommand{\thrI}{\dot{h}^{\im,\bar{r}}}

\newcommand{\hrRk}{\hrR_{\is}}
\newcommand{\hrIk}{\hrI_{\is}}
\newcommand{\thrRk}{\thrR_{\is}}
\newcommand{\thrIk}{\thrI_{\is}}




% n functions: (micro functions)

\newcommand{\na}{\vect{\vn}^{\alpha}}
\newcommand{\tna}{\dot{\vect{\vn}}^{\alpha}}
\newcommand{\nak}{\na_{\is}}
\newcommand{\tnak}{\tna_{\is}}


\newcommand{\nr}{\vect{\vn}^{\bar{r}}}
\newcommand{\tnr}{\dot{\vect{\vn}}^{\bar{r}}}
\newcommand{\nrk}{\nr_{\is}}
\newcommand{\tnrk}{\tnr_{\is}}


%%%% Semi discretized notations:

\newcommand{\SDARk}{\SDvect{A}^{\re}_{\is}}
\newcommand{\SDAIk}{\SDvect{A}^{\im}_{\is}}
\newcommand{\SDAck}{\SDvect{A}^{o}_{\is}}



% Amplitud vector:
\newcommand{\SDAa}{\SDvect{A}^{\alpha}}
\newcommand{\SDAr}{\SDvect{A}^{\bar{r}}}

\newcommand{\SDAak}{\SDAa_{\is}}
\newcommand{\SDArk}{\SDAr_{\is}}





% Admisibility problem:

\newcommand{\SDM}{\SDtens{Q}}
\newcommand{\SDMk}{\SDM}

\newcommand{\SDF}{\SDvect{f}}
\newcommand{\SDFk}{\SDF}



\newcommand{\SDFa}{\SDvect{f}^{\alpha}}
\newcommand{\SDFr}{\SDvect{f}^{\bar{r}}}

\newcommand{\SDFak}{\SDFa_{\is}}
\newcommand{\SDFrk}{\SDFr_{\is}}



% Matrix M (macro):
\newcommand{\SDMa}{\SDtens{Q}^{\alpha}}
\newcommand{\SDMr}{\SDtens{Q}^{\bar{r}}}

\newcommand{\SDMak}{\SDMa_{\is}}
\newcommand{\SDMrk}{\SDMr_{\is}}


% Matrix N (micro)

% For admisibility problem:
\newcommand{\NRk}{\SDtens{N}^{\re}_{\is}}
\newcommand{\NIk}{\SDtens{N}^{\im}_{\is}}

% Preliminary step:
\newcommand{\NRki}{\SDtens{N}^{\re}_{i,\is}}
\newcommand{\NIki}{\SDtens{N}^{\im}_{i,\is}}




\newcommand{\NaRk}{\SDvect{N}^{\re,\alpha}_{\is}}
\newcommand{\NaIk}{\SDvect{N}^{\im,\alpha}_{\is}}
\newcommand{\NrRk}{\SDvect{N}^{\re,\bar{r}}_{\is}}
\newcommand{\NrIk}{\SDvect{N}^{\im,\bar{r}}_{\is}}




% Vectors Coeficients micro:

\newcommand{\ca}{a_{\is}}
\newcommand{\cb}{b_{\is}}

\newcommand{\cau}{a^{(\is)}_{i,\is}}
\newcommand{\cbu}{b^{(\is)}_{i,\is}}




\newcommand{\vcRk}{\SDvect{a}}
\newcommand{\vcIk}{\SDvect{b}_{\is}}

% Preliminary step:
\newcommand{\vcRki}{\SDvect{a}_{i,\is}}
\newcommand{\vcIki}{\SDvect{b}_{i,\is}}



\newcommand{\vcaRk}{\SDvect{a}^{\alpha}_{\is}}
\newcommand{\vcaIk}{\SDvect{b}^{\alpha}_{\is}}

\newcommand{\vcrRk}{\SDvect{a}^{\bar{r}}_{\is}}
\newcommand{\vcrIk}{\SDvect{b}^{\bar{r}}_{\is}}




%%% Preliminary step matrices and vectors:

% semi discretized amplitud macro update:
\newcommand{\SDAup}{\SDvect{A}}


\newcommand{\SDAupk}{\SDvect{A}_{\up,\is}}
\newcommand{\SDMupk}{\SDtens{Q}_{\up,\is}}
\newcommand{\SDFupk}{\SDvect{f}_{\up,\is}}


%% Internal variables:

% Alpha:
\newcommand{\SDAupka}{\SDvect{A}^{\alpha}_{\up,\is}}
\newcommand{\SDMupka}{\SDtens{Q}^{\alpha}_{\up,\is}}
\newcommand{\SDFupka}{\SDvect{f}^{\alpha}_{\up,\is}}


% rbar:
\newcommand{\SDAupkrbar}{\SDvect{A}^{\bar{r}}_{\up,\is}}

\newcommand{\SDMupkrbar}{\SDtens{Q}^{\bar{r}}_{\up,\is}}
\newcommand{\SDFupkrbar}{\SDvect{f}^{\bar{r}}_{\up,\is}}




%%%%%% End Multi scale LATIN





%%%% Hyper reduction method:

\newcommand{\frt}{a_{t}
}
\newcommand{\frs}{a_{s}
}



\newcommand{\redh}[1]{\bar{#1}}

% Reference points 

\newcommand{\ntg}{\Npgt}
\newcommand{\nsg}{n_{s,g}}

\newcommand{\nrt}{\redh{n}_{t,g}}
\newcommand{\nrs}{\redh{n}_{s,g}}


% Indicator points:
\newcommand{\nit}{\redh{\redh{n}}_{t,g}}
\newcommand{\nis}{\redh{\redh{n}}_{s,g}}



% Function case:

% Local Space functions:
\newcommand{\SL}{\Theta}

% Local Time functions
\newcommand{\TLd}{\gamma}
\newcommand{\TLi}{\eta}
\newcommand{\TTLi}{\eta^{up}}
\newcommand{\TL}{\mu}


% POD compressed modes considered:
\newcommand{\nmr}{m_{r}}



% 1) Local Space functions:
\newcommand{\SLF}{\Theta} % Spatial Local Function
%\kappa

\newcommand{\SLp}{\ctens{\SLF}^{p}}
\newcommand{\SLa}{\ctens{\SLF}^{\alpha}}
\newcommand{\SLr}{\SLF^{\bar{r}}}



\newcommand{\SLpd}{\ctens{\redh{\SLF}}^{p}}
\newcommand{\SLad}{\ctens{\redh{\SLF}}^{\alpha}}
\newcommand{\SLrd}{\redh{\SLF}^{\bar{r}}}




% 2) Local Time functions (space reference points):
\newcommand{\TLpd}{\redh{\TL}}
\newcommand{\TLad}{\redh{\TL}^{\alpha}}
\newcommand{\TLrd}{\redh{\TL}^{\bar{r}}}



% 3) Local Time functions (interpolated) 
\newcommand{\TLpi}{\TLi}
\newcommand{\TLai}{\TLi^{\alpha}}
\newcommand{\TLri}{\TLi^{\bar{r}}}

% Time function actualization:
\newcommand{\TTLpi}{\eta^{up}}
\newcommand{\TTLai}{\eta^{\alpha,up}}
\newcommand{\TTLri}{\eta^{\bar{r},up}}


% 4) Local Time functions (Final ones) 
\newcommand{\TLp}{\TL}
\newcommand{\TLa}{\TL^{\alpha}}
\newcommand{\TLr}{\TL^{\bar{r}}}


%%%% End Hyper reduction method:





%% Parallel strategy for the LATIN-PGD method:

% Transmissor operator:

\newcommand{\Tr}{P}
\newcommand{\U}{U}
\newcommand{\Sig}{\Sigma}  
\newcommand{\V}{V}


% patch index nomenclature:
\newcommand{\patchind}{{p}} 

% index of the temp fem element on the patch
\newcommand{\kp}{k_{\patchind}} 
\newcommand{\kN}{k_{\NTpatch}} 



% Domain in time of a given patch
\newcommand{\DTp}{\DT_{\patchind}} 

% temporal elements inside the uniforms patchs in time.
%\newcommand{\nTp}{n_{\prth{T,\patchind}}} 
\newcommand{\nTp}{N_{T}^{(\patchind)}} 
\newcommand{\nTN}{N_{T}^{(\NTpatch)}} 



% temporal elements inside a given patch:
%\newcommand{\nTi}[1]{n_{\prth{T,{#1}}}}
\newcommand{\nTi}[1]{N_{T}^{({#1})}}


\newcommand{\NTpatch}{N} % Patchs in time.


\newcommand{\mi}{\ell} % iteration of the parallel strategy.






%% End Parallel strategy for the LATIN-PGD method:



